Robust Human Registration with Body Part Segmentation on Noisy Point Clouds

Registering human meshes to 3D point clouds is essential for applications such as augmented reality and human-robot interaction but often yields imprecise results due to noise and background clutter in real-world data. We introduce a hybrid approach that incorporates body-part segmentation into the mesh fitting process, enhancing both human pose estimation and segmentation accuracy. Our method first assigns body part labels to individual points, which then guide a two-step SMPL-X fitting: initial pose and orientation estimation using body part centroids, followed by global refinement of the point cloud alignment. Additionally, we demonstrate that the fitted human mesh can refine body part labels, leading to improved segmentation. Evaluations on the cluttered and noisy real-world datasets InterCap, EgoBody, and BEHAVE show that our approach significantly outperforms prior methods in both pose estimation and segmentation accuracy. Code and results are available on our project website: https://segfit.github.io

==> figures/datasets.tex <==
\begin{figure*}[]
    \centering
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[height=3cm]{images/poseprior_visu.png}
        \subcaption{PosePrior}
    \end{minipage}
    \hfill
    % Second image
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[height=3cm]{images/behave_visu.png} % Same height as the others
        \subcaption{BEHAVE}
    \end{minipage}
    \hfill
    % Third image
    \begin{minipage}{0.24\textwidth}
        \centering        \includegraphics[height=3cm]{images/egobody_cropped_visu.png} % Same height as the others
        \subcaption{EgoBody}
    \end{minipage}
    \hfill
    % Fourth image
    \begin{minipage}{0.24\textwidth}
        \centering        \includegraphics[height=3cm]{images/hi4d_visu.png} % Same height as the others
        \subcaption{Hi4D}
    \end{minipage}
    \caption{Examples of point clouds from the datasets used in this study, illustrating variations in pose, occlusions, and interactions present in the PosePrior (AMASS), BEHAVE, EgoBody, and Hi4D datasets. \todo{remove this?}}
    \label{fig:datasets}
\end{figure*}


==> figures/segmentation.tex <==
\begin{figure*}[h]
    \centering
    \begin{minipage}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/segmentation_gt.png}
        \subcaption{Ground Truth}
        \label{fig:ground_truth}
    \end{minipage}
    \hspace{0.05\textwidth}
    \begin{minipage}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/segmentation_original_highlighted.png}
        \subcaption{Human3D}
        \label{fig:original}
    \end{minipage}    
    \hspace{0.05\textwidth}    
    \begin{minipage}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/segmentation_segfit.png}
        \subcaption{SegFit (Ours)}
        \label{fig:segfit}
    \end{minipage}
    \hspace{0.05\textwidth}
    \begin{minipage}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/segmentation_finetuned.png}
        \subcaption{Finetuned}
        \label{fig:finetuned}
    \end{minipage}    
    \caption{Body part segmentation of a scan from the EgoBody dataset, as predicted by Human3D \citep{Takmaz_2023_ICCV} before finetuning (\ref{fig:original}), our proposed method SegFit (\ref{fig:segfit}), and Human3D after finetuning on the pseudo ground truths provided by SegFit (\ref{fig:finetuned}). The arrows in (\ref{fig:original}) highlight how Human3D's separation of body parts was originally imprecise and was corrected by SegFit.}
    \label{fig:segmentation_egobody}
\end{figure*}


==> sections/06_other_stuff.tex <==
\begin{table}[H]
\centering
\scriptsize
\caption{Video Fitting}
\begin{tabular} {l@{\hskip 8pt}ccccc@{\hskip 8pt}}
\toprule
\textbf{Metric} & \textbf{Dance} & \textbf{Fight} & \textbf{Pose} & \textbf{Sidehug} & \textbf{Weighted Average} \\
\midrule
\textbf{Sequential} \\
\text{Time [s]} & 1.482 & 1.965 & 1.286 & 1.730 & 1.622 \\
\text{V2V [mm]} & 20.3 & 25.8 & 21.7 & 27.1 & 23.8 \\
\text{J2J [mm]} & 19.5 & 21.2 & 18.1 & 22.0 & 20.3 \\
\midrule
\textbf{Individual} \\
\text{Time [s]} & 1.852 & 1.989 & 1.768 & 1.723 & 1.827 \\
\text{V2V [mm]} & 21.1 & 24.1 & 22.6 & 29.9 & 24.7 \\
\text{J2J [mm]} & 19.7 & 19.8 & 19.5 & 23.4 & 20.8 \\
\midrule
\textbf{Number of Humans} & 56 & 42 & 38 & 58 & - \\
\bottomrule
\end{tabular}
\label{tab:video_fitting}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/untitled.png}
\end{figure}

==> tables/finetuning.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l@{\hskip 8pt}cccccc@{\hskip 8pt}}
\toprule
\textbf{Human3D Model} & \textbf{Metric} & \textbf{BEHAVE} & \textbf{Intercap} \\
\midrule
w/o Fine-Tuning & \multirow{2}{*}{Accuracy} & $74.61$\% & $55.85$\% \\
w/\phantom{ } Fine-Tuning & & $\mathbf{89.96}$\% & $\mathbf{67.98}$\% \\
\midrule
w/o Fine-Tuning & \multirow{2}{*}{IoU} & $57.38$\% & $45.37$\%\\
w/\phantom{ } Fine-Tuning & & $\mathbf{75.36}$\% & $\mathbf{56.71}$\% \\
\midrule
w/o Fine-Tuning & \multirow{2}{*}{mAP} & $73.42$\% & $59.54$\%\\
w/\phantom{ } Fine-Tuning & & $\mathbf{84.56}$\% & $\mathbf{68.18}$\% \\
\bottomrule
\end{tabular}
\vspace{-5px}
\caption{Segmentation performance of Human3D~\citep{Takmaz_2023_ICCV} before and after fine-tuning on the outputs of the proposed SegFit.}
\label{tab:finetuning_improvements}
\end{table}

% \begin{table*}[h]
% \centering
% \begin{tabular}{l@{\hskip 8pt}cccccc@{\hskip 8pt}}
% \toprule
% \textbf{Human3D Model} & \textbf{Metric} & \textbf{BEHAVE} & \textbf{EgoBody} & \textbf{Intercap} \\
% \midrule
% w/o Fine-Tuning & \multirow{2}{*}{Accuracy} & 74.61\% & 77.06\% & 55.85\% \\
% w/\phantom{ } Fine-Tuning & & \textbf{89.96}\% & \textbf{86.28}\% & \textbf{67.98\%} \\
% \midrule
% w/o Fine-Tuning & \multirow{2}{*}{IoU} & 57.38\% & 62.89\% & 45.37\%\\
% w/\phantom{ } Fine-Tuning & & \textbf{75.36}\% & \textbf{71.16}\% & 56.71\% \\
% \midrule
% w/o Fine-Tuning & \multirow{2}{*}{mAP} & 73.42\% & 73.98\% & 59.54\%\\
% w/\phantom{ } Fine-Tuning & & \textbf{84.56}\% & \textbf{78.07}\% & 68.18\% \\
% \bottomrule
% \end{tabular}
% \caption{Segmentation performance of Human3D~\citep{Takmaz_2023_ICCV} before and after fine-tuning in a self-supervised manner on the outputs of the proposed SegFit.}
% \label{tab:finetuning_improvements}
% \end{table*}
